Benchmark for Anonymous Video Analytics

Out-of-home audience measurement aims to count and characterize the people exposed to advertising content in the physical world. While audience measurement solutions based on computer vision are of increasing interest, no commonly accepted benchmark exists to evaluate and compare their performance. In this paper, we propose the first benchmark for digital out-of-home audience measurement that evaluates the vision-based tasks of audience localization and counting, and audience demographics. The benchmark is composed of a novel, dataset captured at multiple locations and a set of performance measures. Using the benchmark, we present an in-depth comparison of eight open-source algorithms on four hardware platforms with GPU and CPU-optimized inferences and of two commercial off-the-shelf solutions for localization, count, age, and gender estimation. This benchmark and related open-source codes are available at http://ava.eecs.qmul.ac.uk.

==> results_per_sequence_S1_video0.tex <==
Frame	actInst	actCum	estInst0	estCum0	estInst1	estCum1	estInst2	estCum2	estInst3	estCum3
0	2	0	6	0	0	0	0	0	0	0
30	2	3	3	137	0	0	3	5	4	5
60	3	4	3	291	0	0	3	6	4	7
90	2	4	4	461	0	2	1	6	4	7
120	3	6	5	635	1	2	2	6	5	8
150	4	7	3	798	0	7	2	6	4	8
180	4	7	3	944	0	7	3	7	6	10
210	4	7	7	1133	1	8	4	8	6	10
240	3	7	5	1281	2	53	4	8	5	10
270	3	7	5	1420	0	75	6	10	6	11
300	3	7	6	1577	1	99	6	10	6	11
330	3	7	7	1752	1	128	6	10	6	11
360	3	7	8	1938	1	159	5	10	6	11
390	3	7	8	2160	2	189	5	10	6	11
420	3	7	8	2363	2	251	4	10	5	11
450	3	7	12	2574	2	320	5	11	6	12
480	3	7	9	2843	2	396	5	11	5	12
510	4	7	6	3084	2	456	5	11	6	12
540	3	7	4	3241	2	516	4	11	5	12
570	3	7	3	3395	2	576	4	11	5	12
600	3	7	4	3493	1	630	2	11	3	12
630	3	7	3	3631	1	683	3	11	3	13
660	2	7	1	3691	1	720	1	11	1	14
690	1	7	1	3721	1	750	1	11	1	14
720	1	7	1	3752	1	780	1	11	1	14
750	1	7	1	3783	1	810	1	11	1	14
780	1	7	1	3815	1	840	1	11	1	14
810	1	7	1	3851	1	870	1	11	1	14
840	1	7	1	3882	1	900	1	11	1	14
870	1	7	0	3904	0	917	0	11	0	14
900	0	7	0	3905	0	917	0	11	0	14
930	0	7	0	3905	0	917	0	11	0	14
960	0	7	0	3905	0	917	0	11	0	14
990	0	7	0	3905	0	917	0	11	0	14
1020	0	7	0	3905	0	917	0	11	0	14
1050	0	7	0	3905	0	917	0	11	0	14
1080	0	7	1	3907	0	917	0	11	0	14
1110	0	7	1	3937	0	917	0	11	0	14
1140	0	7	0	3949	0	917	0	11	0	14
1170	0	7	0	3949	0	917	0	11	0	14
1200	0	7	1	3949	0	917	0	11	0	14
1230	0	7	0	3954	0	917	0	11	0	14
1260	0	7	0	3954	0	917	0	11	0	14
1290	0	7	0	3954	0	917	0	11	0	14
1320	0	7	0	3954	0	917	0	11	0	14
1350	0	7	0	3955	0	917	0	11	0	14
1380	0	7	0	3955	0	917	0	11	0	14
1410	0	7	1	3959	0	917	0	11	0	14
1440	0	7	0	3965	0	917	0	11	0	14
1470	0	7	0	3968	0	917	0	11	0	14
1500	1	8	2	3991	0	917	1	11	1	15
1530	0	8	1	4007	0	917	1	11	1	15
1560	0	8	0	4022	0	917	1	11	1	15
1590	0	8	0	4026	0	917	1	11	1	15
1620	0	8	0	4026	0	917	1	11	1	15
1650	0	8	0	4026	0	917	1	11	1	15
1680	0	8	0	4028	0	917	1	11	1	15
1710	0	8	0	4029	0	917	1	11	1	15
1740	0	8	1	4036	0	917	1	11	1	15
1770	0	8	1	4065	0	917	1	11	1	15
1800	1	8	1	4099	0	917	1	11	1	15
1830	0	8	0	4102	0	917	0	11	0	15
1860	1	9	0	4102	0	917	0	11	0	15
1890	1	9	0	4105	0	917	0	11	0	15
1920	2	10	0	4109	0	917	0	11	0	15
1950	2	10	1	4125	0	917	1	12	1	16
1980	2	11	1	4157	1	938	1	12	3	18
2010	2	11	1	4191	0	950	1	12	3	18
2040	2	11	2	4261	0	952	1	14	3	18
2070	3	12	3	4321	0	956	1	14	3	18
2100	4	13	2	4387	1	957	2	16	3	19
2130	3	13	3	4465	0	983	1	16	2	19
2160	4	14	1	4518	1	1007	2	16	3	20
2190	3	14	2	4572	1	1037	3	16	3	20
2220	3	14	6	4682	1	1067	4	17	4	21
2250	3	14	6	4792	1	1097	4	17	4	21
2280	4	14	4	4914	1	1127	3	17	3	21
2310	3	14	5	5075	1	1157	3	18	3	21
2340	3	14	3	5197	1	1186	1	18	3	21
2370	3	14	3	5302	1	1216	3	18	3	23
2400	2	14	2	5386	0	1222	2	18	2	23
2430	2	14	5	5496	0	1222	3	18	3	24
2460	2	14	1	5596	0	1237	2	18	2	24
2490	2	14	1	5658	0	1239	1	18	2	24
2520	2	14	3	5727	0	1250	2	18	3	24
2550	2	14	3	5811	1	1265	3	19	3	24
2580	2	14	3	5916	0	1275	3	19	3	24
2610	2	14	3	6031	2	1316	3	19	3	24
2640	2	14	3	6132	2	1375	3	19	3	24
2670	3	14	4	6208	2	1428	3	19	3	24
2700	3	14	4	6328	3	1510	4	20	4	25
2730	3	14	4	6454	3	1600	4	20	4	25
2760	4	14	4	6594	3	1691	4	20	4	25
2790	4	15	4	6732	2	1772	4	20	4	25
2820	4	15	6	6876	3	1852	4	20	4	25
2850	3	15	5	6996	3	1939	3	20	3	25
2880	4	16	4	7144	3	2031	3	20	3	25
2910	4	16	4	7280	2	2102	3	21	3	26
2940	4	16	3	7411	1	2150	3	21	2	27
2970	3	16	2	7494	1	2187	2	21	2	27
3000	2	16	2	7554	1	2206	2	21	2	27
3030	1	16	2	7615	1	2235	2	21	2	27
3060	2	16	2	7677	1	2265	2	21	2	27
3090	2	16	3	7754	1	2305	2	21	2	27
3120	2	16	2	7815	1	2349	1	21	2	27
3150	2	16	2	7876	1	2381	2	21	2	27
3180	1	16	2	7944	1	2413	2	21	2	27
3210	1	16	1	8008	1	2443	2	21	2	27
3240	0	16	1	8046	0	2450	1	21	1	27
3270	0	16	1	8070	0	2450	1	21	1	27
3300	0	16	1	8100	0	2450	1	21	1	27
3330	0	16	1	8131	0	2450	1	21	1	27
3360	1	16	1	8161	0	2450	1	21	1	27
3390	0	16	0	8164	0	2450	0	21	0	27
3420	0	16	0	8164	0	2450	0	21	0	27
3450	0	16	0	8164	0	2450	0	21	0	27
3480	0	16	0	8165	0	2450	0	21	0	27
3510	0	16	0	8165	0	2450	0	21	0	27
3540	0	16	0	8165	0	2450	0	21	0	27
3570	0	16	0	8165	0	2450	0	21	0	27
3600	0	16	0	8165	0	2450	0	21	0	27
3630	0	16	0	8168	0	2450	0	21	0	27
3660	0	16	0	8168	0	2450	0	21	0	27
3690	0	16	0	8168	0	2450	0	21	0	27
3720	0	16	0	8168	0	2450	0	21	0	27
3750	0	16	0	8168	0	2450	0	21	0	27
3780	0	16	1	8169	0	2450	0	21	0	27
3810	1	17	1	8194	1	2453	1	22	1	28
3840	0	17	0	8205	0	2454	1	22	1	28
3870	0	17	0	8211	0	2454	1	22	1	28
3900	0	17	1	8243	0	2454	1	22	1	28
3930	0	17	2	8266	0	2454	1	22	1	28
3960	0	17	1	8292	0	2454	1	22	1	28
3990	0	17	2	8313	0	2454	1	22	1	28
4020	1	18	2	8360	0	2454	2	23	2	29
4050	1	18	3	8430	0	2454	3	24	3	30
4080	1	18	3	8526	0	2454	3	24	3	30
4110	1	18	3	8631	0	2454	3	24	3	30
4140	1	18	3	8736	0	2454	3	24	3	30
4170	1	18	2	8816	0	2454	1	24	2	30
4200	1	18	4	8898	0	2454	2	24	2	31
4230	1	18	4	9017	0	2454	3	24	3	31
4260	2	18	3	9132	0	2454	3	24	3	31
4290	1	18	3	9209	0	2454	2	24	2	31
4320	1	18	2	9307	0	2454	2	24	2	31
4350	1	18	3	9388	0	2454	2	24	2	31
4380	1	18	2	9460	0	2454	2	24	2	31
4410	1	18	1	9548	0	2454	1	24	2	31
4440	1	18	2	9603	0	2454	2	24	2	31
4470	1	18	3	9673	0	2455	2	24	2	31
4500	1	18	3	9745	0	2459	2	24	2	31
4530	1	18	3	9821	0	2464	2	24	2	31
4560	1	18	2	9900	0	2464	2	24	2	31
4590	1	18	2	9978	0	2464	2	24	2	31
4620	1	18	1	10019	0	2464	1	24	1	31
4650	1	18	4	10068	1	2469	2	25	2	32
4680	1	18	3	10154	1	2497	2	25	2	32
4710	1	18	2	10223	1	2527	2	25	2	32
4740	1	18	3	10286	0	2550	2	25	2	32
4770	1	18	2	10378	0	2553	2	25	2	32
4800	1	18	2	10452	0	2556	2	25	2	32
4830	1	18	3	10518	1	2582	2	25	2	32
4860	2	19	2	10572	0	2595	2	25	2	32
4890	3	20	2	10644	0	2595	2	25	2	32
4920	4	21	5	10794	2	2626	4	27	3	33
4950	4	21	5	10945	2	2680	4	27	4	34
4980	4	21	9	11123	1	2724	4	27	4	34
5010	4	21	8	11364	2	2766	4	27	4	34
5040	4	21	7	11554	1	2807	4	27	4	34
5070	2	21	3	11697	1	2848	3	27	3	34
5100	3	21	4	11780	2	2898	2	27	3	35
5130	3	21	4	11884	0	2946	2	27	3	37
5160	3	21	3	11979	1	2979	3	27	4	37
5190	3	21	4	12095	1	3024	3	27	4	37
5220	3	21	6	12218	1	3055	4	28	4	37
5250	2	21	4	12331	1	3085	3	28	3	37
5280	2	21	3	12426	1	3115	3	28	3	37
5310	2	21	5	12537	1	3145	3	28	3	37
5340	1	21	3	12629	0	3150	2	28	2	37
5370	1	21	4	12701	0	3150	2	28	2	37
5400	1	21	1	12745	0	3150	2	28	2	37
5430	1	21	1	12829	0	3150	2	28	2	37
5460	1	21	2	12884	0	3150	2	28	2	37
5490	1	21	2	12936	0	3150	2	28	2	37
5520	2	21	2	12996	0	3150	2	28	2	37
5550	1	21	1	13027	0	3150	1	28	1	37
5580	2	22	3	13078	0	3156	2	28	2	38
5610	2	22	3	13168	1	3176	2	28	2	38
5640	2	22	3	13258	1	3206	3	29	2	38
5670	2	22	4	13348	1	3236	3	29	3	39
5700	2	22	3	13454	1	3266	3	29	3	39
5730	3	23	4	13575	2	3312	3	29	3	39
5760	3	23	3	13673	2	3372	3	29	3	39
5790	3	23	4	13766	2	3431	3	29	3	39
5820	3	23	3	13877	2	3489	3	29	3	39
5850	3	23	3	13991	2	3549	3	29	3	39
5880	3	23	4	14081	2	3609	3	29	3	39
5910	3	23	4	14194	2	3669	2	29	3	39
5940	3	23	5	14292	2	3729	3	29	3	39
5970	3	23	3	14417	2	3790	2	29	2	39
6000	2	23	2	14505	2	3849	2	29	2	40
6030	2	23	2	14565	1	3880	2	29	2	40
6060	2	23	2	14643	0	3907	2	29	2	41
6090	2	23	2	14722	1	3927	3	29	3	42
6120	2	23	2	14787	1	3957	3	29	3	42
6150	2	23	2	14849	1	3987	3	29	3	42
6180	3	24	3	14914	1	4017	3	29	3	42
6210	3	24	4	15007	1	4047	4	30	4	43
6240	3	24	3	15119	2	4092	4	30	4	43
6270	3	24	5	15262	1	4142	4	30	4	43
6300	3	24	4	15401	1	4185	4	30	4	43
6330	3	24	4	15533	1	4221	4	30	4	43
6360	4	25	4	15659	2	4269	4	30	4	43
6390	4	25	5	15779	1	4309	3	30	3	43
6420	3	25	3	15892	2	4356	3	30	3	43
6450	4	26	4	16002	4	4419	4	30	4	44
6480	5	26	5	16146	3	4498	5	31	5	45
6510	5	26	6	16344	3	4557	5	31	5	45
6540	5	26	5	16501	2	4654	5	31	5	45
6570	5	26	7	16673	4	4748	5	31	5	45
6600	5	26	5	16858	2	4853	4	31	4	45
6630	4	26	5	17025	4	4952	4	31	4	45
6660	4	26	5	17215	3	5051	4	31	4	45
6690	4	26	4	17358	4	5152	4	31	4	46
6720	4	26	5	17519	3	5255	4	31	5	46
6750	4	26	5	17659	4	5371	4	31	4	46
6780	4	26	3	17794	3	5456	3	31	3	46
6810	3	26	3	17910	2	5542	2	31	2	48
6840	2	26	2	17978	2	5602	2	31	2	48
6870	2	26	2	18039	2	5660	2	31	2	48
6900	2	26	2	18103	2	5721	2	31	2	48
6930	3	27	2	18164	2	5782	2	31	2	48
6960	3	27	3	18226	1	5822	2	31	2	50
6990	1	27	2	18287	1	5852	2	31	2	50
7020	1	27	3	18350	1	5882	2	31	2	50
7050	1	27	1	18414	1	5912	2	31	2	50
7080	1	27	1	18473	1	5942	2	31	2	50
7110	1	27	1	18528	1	5972	2	31	2	50
7140	1	27	2	18588	1	6002	2	31	2	50
7170	1	27	2	18627	1	6032	2	31	2	50
7200	1	27	3	18680	1	6062	2	31	2	50
7230	1	27	1	18742	1	6092	2	31	2	50
7260	1	27	4	18814	1	6122	2	31	2	50
7290	1	27	2	18886	1	6152	2	31	2	50
7320	1	27	2	18953	1	6182	2	31	2	50
7350	1	27	2	19019	1	6212	2	31	2	50
7380	2	27	1	19054	1	6242	2	31	2	50
7410	1	27	1	19084	1	6272	1	31	1	50
7440	1	27	1	19115	1	6302	1	31	1	50
7470	1	27	2	19147	1	6332	1	31	1	50
7500	1	27	1	19178	1	6362	1	31	1	50
7530	1	27	1	19208	1	6392	1	31	1	50
7560	1	27	1	19238	1	6422	1	31	1	50
7590	1	27	1	19268	1	6452	1	31	1	50
7620	1	27	1	19298	1	6482	1	31	1	50
7650	1	27	1	19329	1	6512	1	31	1	50
7680	1	27	1	19359	1	6542	1	31	1	50
7710	1	27	1	19389	1	6572	1	31	1	50
7740	1	27	1	19419	1	6602	1	31	1	50
7770	1	27	1	19449	1	6632	1	31	1	50
7800	2	27	2	19492	2	6668	2	32	2	51
7830	2	27	2	19552	2	6728	2	32	2	51
7860	2	27	2	19628	2	6788	2	33	2	52
7890	2	27	2	19687	1	6825	2	33	2	52
7920	2	27	1	19723	1	6855	2	33	2	52
7950	2	27	1	19753	1	6885	2	33	2	52
7980	2	27	2	19787	1	6915	3	34	3	53
8010	2	27	2	19854	2	6963	3	34	3	53
8040	2	27	2	19921	2	7023	3	34	3	53
8070	2	27	2	19998	2	7083	3	34	3	53
8100	1	27	3	20069	1	7121	3	34	3	53
8130	1	27	2	20136	1	7151	2	34	2	54
8160	1	27	3	20208	1	7181	3	35	3	56
8190	1	27	1	20270	0	7209	3	35	3	56
8220	0	27	1	20301	0	7209	2	35	2	56
8250	0	27	2	20353	0	7209	2	35	2	56
8280	0	27	2	20415	0	7209	2	35	2	56
8310	0	27	1	20467	0	7210	2	35	2	56
8340	0	27	3	20512	0	7212	2	35	2	56
8370	0	27	1	20542	0	7212	1	35	2	56
8400	0	27	2	20577	0	7212	2	36	2	56
8430	1	27	2	20624	0	7212	1	36	2	56
8460	1	27	0	20647	0	7212	0	36	0	56
8490	0	27	0	20647	0	7212	0	36	0	56
8520	0	27	0	20647	0	7212	0	36	0	56
8550	0	27	0	20647	0	7212	0	36	0	56
8580	0	27	0	20647	0	7212	0	36	0	56
8610	0	27	0	20647	0	7212	0	36	0	56
8640	0	27	0	20647	0	7212	0	36	0	56
8670	0	27	1	20653	0	7212	1	37	1	57
8700	0	27	1	20686	0	7212	1	37	1	57
8730	0	27	1	20717	0	7212	1	37	1	57
8760	0	27	2	20747	0	7212	1	37	1	57
8790	0	27	1	20778	0	7212	1	37	1	57
8820	1	28	2	20814	0	7212	1	37	1	57
8850	1	28	2	20850	0	7212	1	37	1	57
8880	1	28	1	20889	0	7212	1	37	1	57
8910	1	28	1	20919	0	7212	1	37	1	57
8940	1	28	1	20953	0	7212	1	37	1	57
8970	1	28	1	20983	0	7212	1	37	1	57
9000	1	28	1	21013	0	7212	1	37	1	57
9030	1	29	1	21046	0	7212	2	38	2	58
9060	1	29	2	21097	0	7212	2	38	2	58
9090	1	29	2	21157	0	7212	2	38	2	58
9120	1	29	1	21214	0	7212	1	38	1	58
9150	1	29	1	21245	0	7212	1	38	2	58
9180	1	29	1	21276	0	7212	2	38	2	58
9210	1	29	2	21308	0	7212	2	38	2	58
9240	1	29	2	21342	0	7212	2	38	2	58
9270	1	29	2	21389	0	7212	2	38	2	58
9300	1	29	2	21443	0	7212	2	38	2	58
9330	1	29	2	21503	0	7213	2	38	2	58
9360	1	29	2	21563	0	7213	2	38	2	58
9390	1	29	1	21618	0	7218	2	38	2	58
9420	1	29	1	21670	0	7218	2	38	2	58
9450	1	29	2	21717	0	7223	2	38	2	58
9480	1	29	3	21785	0	7223	2	38	2	59
9510	0	29	6	21847	0	7223	2	39	3	60
9540	0	29	3	21931	0	7223	3	39	3	60
9570	0	29	2	22031	0	7223	2	39	3	60
9600	0	29	5	22150	0	7223	1	39	3	60
9630	0	29	6	22268	0	7223	1	39	3	60
9660	0	29	2	22377	0	7223	1	39	3	60
9690	0	29	3	22439	0	7223	0	39	2	60
9720	0	29	4	22521	0	7223	0	39	2	60
9750	0	29	3	22599	0	7223	0	39	2	60
9780	0	29	3	22682	0	7223	0	39	2	60
9810	0	29	0	22752	0	7223	1	39	2	60
9840	0	29	0	22752	0	7223	0	39	1	60
9870	0	29	0	22752	0	7223	0	39	1	60
9900	0	29	0	22752	0	7223	0	39	0	60
9930	0	29	0	22752	0	7223	0	39	0	60
9960	0	29	0	22752	0	7223	0	39	0	60
9990	0	29	0	22752	0	7223	0	39	0	60

